P-CRITICAL: A Reservoir Autoregulation Plasticity Rule for Neuromorphic Hardware

Backpropagation algorithms on recurrent artificial neural networks require an unfolding of accumulated states over time. These states must be kept in memory for an undefined period of time which is task-dependent. This paper uses the reservoir computing paradigm where an untrained recurrent neural network layer is used as a preprocessor stage to learn temporal and limited data. These so-called reservoirs require either extensive fine-tuning or neuroplasticity with unsupervised learning rules. We propose a new local plasticity rule named P-CRITICAL designed for automatic reservoir tuning that translates well to Intel's Loihi research chip, a recent neuromorphic processor. We compare our approach on well-known datasets from the machine learning community while using a spiking neuronal architecture. We observe an improved performance on tasks coming from various modalities without the need to tune parameters. Such algorithms could be a key to end-to-end energy-efficient neuromorphic-based machine learning on edge devices.

==> discussion.tex <==
When validating the model, it is clear that P-CRITICAL achieved its goal by tuning the branching factor of various reservoirs. The algorithm was able to offer a stable activity when connected to various raw input spike trains. By doing so, we believe that the reservoir offers maximal activity and memory retention without suffering from sub or super criticality. The plasticity rule was able to increase the test accuracy of unoptimized reservoirs for various high-level tasks coming from different sensory inputs that were captured with event-based sensors. We aim for P-CRITICAL to offer a "one-model fits all", such that it can be implemented on a neuromorphic processor and offer low-power edge devices the ability to train without requiring extensive computation or cloud server access. Reservoir computing is a good alternative to RNNs for faster training times, and plasticity-enabled reservoirs are well suited for neuromorphic engineering applications as they are slow on conventional computer architecture. This is because plasticity rules often prevent batching of the input data while the recurrent dynamics of reservoirs forces sequential simulations.


